Conformal Prediction for Time Series with Modern Hopfield Networks

To quantify uncertainty, conformal prediction methods are gaining continuously more interest and have already been successfully applied to various domains. However, they are difficult to apply to time series as the autocorrelative structure of time series violates basic assumptions required by conformal prediction. We propose HopCPT, a novel conformal prediction approach for time series that not only copes with temporal structures but leverages them. We show that our approach is theoretically well justified for time series where temporal dependencies are present. In experiments, we demonstrate that our new approach outperforms state-of-the-art conformal prediction methods on multiple real-world time series datasets from four different domains.

==> _arxiv/main_arxiv_v2.tex <==
\input{main_icml_v2}

==> other_tables/hyperparameter.tex <==
\begin{table}[h]
\centering
\caption{Parameters used in the hyperparameter search.}
\label{tab:hyperparameter-grid}
\vskip 0.15in
\begin{tabular}{@{}lll@{}}
\toprule
Method & Parameter & Value \\ \midrule
\multirow{3}{*}{\ourmethod}  & Learning Rate & 0.01, 0.001  \\
                             & Dropout       & 0, 0.25, 0.5 \\ 
                             & Time Encode   & yes/no  
                             \\ \midrule
\multirow{2}{*}{\adaptiveci} & Mode          & simple, momentum  \\
                             & $\gamma$      & 0.002, 0.005, 0.01, 0.02    \\ \midrule
\enbpi                       & Window Length & \begin{tabular}[c]{@{}l@{}}200, 150, 125, 100,\\ 75, 50, 25, 10\end{tabular}          \\ \midrule
\nexcp                       & $\rho$        & \begin{tabular}[c]{@{}l@{}}0.999, 0.995, 0.993,\\ 0.99, 0.98, 0.95, 0.90\end{tabular} \\ \midrule
\knn                       & k-Top Share        & \begin{tabular}[c]{@{}l@{}}0.025, 0.05, 0.10, 0.15, \\ 0.20, 0.25, 0.30, 0.35\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}


==> results_tables/rolling_coverage_bak.tex <==
% -------------
    %!!!
    %DO NOT MANUALLY CHANGE THE ENTRIES BELOW - TABLE AND COMMENTS ARE AUTOGENERATED 
    %!!!
    %If you see a general problem talk to Andreas he can adapt the code for the generation
    %If you really have to make a manual change then add a comment in results/manual_change.txt so that we can
    %redo the change if a new table version is generated

%Dataset:
%Comment:None

\begin{table}
\centering
\caption{\nextTableCaption}
\label{tab:rolling-coverage}
\small
\begin{tabular}{llllllll}
\toprule
 &  & UC & \rotatebox{90}{\ourmethod} & \rotatebox{90}{SPIC} & \rotatebox{90}{EnbPI} & \rotatebox{90}{NexCP} & \rotatebox{90}{CP} \\
Data & FC & Window &  &  &  &  &  \\
\midrule
\multirow[c]{9}{*}{\rotatebox{90}{Solar Small}} & \multirow[c]{3}{*}{\rotatebox{90}{Forest}} & 10 & $.74$ & $.57$ & $.67$ & $.67$ & $.69$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.70$ & $.34$ & $.56$ & $.53$ & $.54$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.66$ & $.15$ & $.52$ & $.46$ & $.48$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{LGBM}} & 10 & $.72$ & $.59$ & $.66$ & $.67$ & $.68$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.66$ & $.43$ & $.53$ & $.54$ & $.57$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.59$ & $.26$ & $.46$ & $.45$ & $.46$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{Ridge}} & 10 & $.72$ & $.59$ & $.66$ & $.74$ & $.72$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.65$ & $.46$ & $.57$ & $.65$ & $.61$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.55$ & $.26$ & $.47$ & $.58$ & $.54$ \\
\cline{1-8} \cline{2-8}
\multirow[c]{9}{*}{\rotatebox{90}{Solar 1Y}} & \multirow[c]{3}{*}{\rotatebox{90}{Forest}} & 10 & $.87$ & $.87$ & $.67$ & $.71$ & $.90$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.86$ & $.87$ & $.56$ & $.64$ & $.88$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.86$ & $.87$ & $.46$ & $.61$ & $.89$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{LGBM}} & 10 & $.75$ & $.87$ & $.68$ & $.72$ & $.91$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.69$ & $.87$ & $.57$ & $.64$ & $.89$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.65$ & $.87$ & $.47$ & $.61$ & $.91$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{Ridge}} & 10 & $.69$ & $.84$ & $.64$ & $.70$ & $.68$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.64$ & $.81$ & $.54$ & $.62$ & $.61$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.58$ & $.79$ & $.41$ & $.56$ & $.56$ \\
\cline{1-8} \cline{2-8}
\multirow[c]{9}{*}{\rotatebox{90}{Solar 3Y}} & \multirow[c]{3}{*}{\rotatebox{90}{Forest}} & 10 & $.82$ & - & $.65$ & $.71$ & $.75$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.79$ & - & $.52$ & $.63$ & $.65$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.78$ & - & $.38$ & $.57$ & $.59$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{LGBM}} & 10 & $.75$ & - & $.67$ & $.71$ & $.75$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.70$ & - & $.55$ & $.63$ & $.66$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.65$ & - & $.43$ & $.57$ & $.59$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{Ridge}} & 10 & $.86$ & - & $.51$ & $.73$ & $.76$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.85$ & - & $.33$ & $.65$ & $.68$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.86$ & - & $.09$ & $.59$ & $.62$ \\
\cline{1-8} \cline{2-8}
\multirow[c]{9}{*}{\rotatebox{90}{Air 10 PM}} & \multirow[c]{3}{*}{\rotatebox{90}{Forest}} & 10 & $.82$ & $.81$ & $.69$ & $.79$ & $.79$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.80$ & $.78$ & $.62$ & $.74$ & $.75$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.78$ & $.75$ & $.50$ & $.66$ & $.69$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{LGBM}} & 10 & $.79$ & $.83$ & $.69$ & $.79$ & $.78$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.76$ & $.81$ & $.62$ & $.73$ & $.74$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.73$ & $.79$ & $.51$ & $.66$ & $.69$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{Ridge}} & 10 & $.78$ & $.83$ & $.70$ & $.78$ & $.84$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.74$ & $.80$ & $.62$ & $.72$ & $.80$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.70$ & $.78$ & $.51$ & $.65$ & $.76$ \\
\cline{1-8} \cline{2-8}
\multirow[c]{9}{*}{\rotatebox{90}{Air 25 PM}} & \multirow[c]{3}{*}{\rotatebox{90}{Forest}} & 10 & - & $.77$ & $.69$ & $.79$ & $.78$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & - & $.73$ & $.61$ & $.73$ & $.73$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & - & $.70$ & $.50$ & $.64$ & $.66$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{LGBM}} & 10 & $.67$ & $.78$ & $.69$ & $.80$ & $.77$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.60$ & $.74$ & $.61$ & $.74$ & $.71$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.51$ & $.71$ & $.50$ & $.67$ & $.64$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{Ridge}} & 10 & $.72$ & $.79$ & $.69$ & $.79$ & $.81$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.66$ & $.76$ & $.62$ & $.73$ & $.78$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.59$ & $.72$ & $.50$ & $.65$ & $.71$ \\
\cline{1-8} \cline{2-8}
\multirow[c]{9}{*}{\rotatebox{90}{Sap flow}} & \multirow[c]{3}{*}{\rotatebox{90}{Forest}} & 10 & $.73$ & $.80$ & $.74$ & $.82$ & $.84$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.68$ & $.77$ & $.67$ & $.77$ & $.79$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.61$ & $.73$ & $.56$ & $.69$ & $.73$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{LGBM}} & 10 & $.62$ & $.80$ & $.74$ & $.81$ & $.82$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.54$ & $.75$ & $.67$ & $.76$ & $.75$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.44$ & $.72$ & $.56$ & $.67$ & $.69$ \\
\cline{2-8}
\rotatebox{90}{} & \multirow[c]{3}{*}{\rotatebox{90}{Ridge}} & 10 & $.69$ & $.56$ & $.72$ & $.79$ & $.47$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 20 & $.62$ & $.50$ & $.63$ & $.73$ & $.43$ \\
\rotatebox{90}{} & \rotatebox{90}{} & 50 & $.53$ & $.42$ & $.49$ & $.63$ & $.37$ \\
\cline{1-8} \cline{2-8}
\bottomrule
\end{tabular}
\end{table}


==> results_tables/spic_length_comparsion.tex <==
% -------------
    %!!!
    %DO NOT MANUALLY CHANGE THE ENTRIES BELOW - TABLE AND COMMENTS ARE AUTOGENERATED 
    %!!!
    %If you see a general problem talk to Andreas he can adapt the code for the generation
    %If you really have to make a manual change then add a comment in results/manual_change.txt so that we can
    %redo the change if a new table version is generated

%Dataset:
%Comment:None

\begin{table}
\centering
\caption{\nextTableCaption}
\label{tab:spic-length-comparsion}
\vskip 0.15in
\small
\begin{tabular}{lllS[separate-uncertainty, table-alignment-mode=none]S[separate-uncertainty, table-alignment-mode=none]}
\toprule
 &  & Window & 100 & 25 \\
Data & FC &  &  &  \\
\midrule
\multirow[c]{9}{*}{\rotatebox{90}{Solar 1Y}} & \multirow[c]{3}{*}{Forest} & $\Delta$ Cov & $0.045^{\pm 0.000}$ & $0.047^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $97.2^{\pm 0.1}$ & $97.8^{\pm 0.3}$ \\
\rotatebox{90}{} &  & Winkler & $1.26^{\pm 0.00}$ & $1.25^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{LGBM} & $\Delta$ Cov & $0.045^{\pm 0.000}$ & $0.047^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $96.6^{\pm 0.2}$ & $97.6^{\pm 0.1}$ \\
\rotatebox{90}{} &  & Winkler & $1.26^{\pm 0.00}$ & $1.26^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{Ridge} & $\Delta$ Cov & $0.031^{\pm 0.000}$ & $0.030^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $112.9^{\pm 0.2}$ & $113.7^{\pm 0.1}$ \\
\rotatebox{90}{} &  & Winkler & $1.40^{\pm 0.00}$ & $1.42^{\pm 0.00}$ \\
\cmidrule{1-5}
\multirow[c]{9}{*}{\rotatebox{90}{Solar Small}} & \multirow[c]{3}{*}{Forest} & $\Delta$ Cov & $-0.064^{\pm 0.002}$ & $-0.024^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $38.8^{\pm 0.4}$ & $43.2^{\pm 0.2}$ \\
\rotatebox{90}{} &  & Winkler & $1.82^{\pm 0.01}$ & $1.53^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{LGBM} & $\Delta$ Cov & $-0.052^{\pm 0.002}$ & $-0.027^{\pm 0.001}$ \\
\rotatebox{90}{} &  & PI-Width & $37.4^{\pm 0.2}$ & $43.3^{\pm 0.1}$ \\
\rotatebox{90}{} &  & Winkler & $1.84^{\pm 0.01}$ & $1.63^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{Ridge} & $\Delta$ Cov & $-0.055^{\pm 0.002}$ & $-0.057^{\pm 0.001}$ \\
\rotatebox{90}{} &  & PI-Width & $51.9^{\pm 0.2}$ & $52.8^{\pm 0.2}$ \\
\rotatebox{90}{} &  & Winkler & $1.91^{\pm 0.02}$ & $1.83^{\pm 0.00}$ \\
\cmidrule{1-5}
\multirow[c]{9}{*}{\rotatebox{90}{Air 10 PM}} & \multirow[c]{3}{*}{Forest} & $\Delta$ Cov & $0.008^{\pm 0.000}$ & $0.008^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $118.5^{\pm 0.0}$ & $118.5^{\pm 0.1}$ \\
\rotatebox{90}{} &  & Winkler & $2.23^{\pm 0.00}$ & $2.23^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{LGBM} & $\Delta$ Cov & $0.024^{\pm 0.000}$ & $0.023^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $113.2^{\pm 0.2}$ & $113.2^{\pm 0.1}$ \\
\rotatebox{90}{} &  & Winkler & $1.94^{\pm 0.00}$ & $1.94^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{Ridge} & $\Delta$ Cov & $0.024^{\pm 0.000}$ & $0.024^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $93.9^{\pm 0.0}$ & $93.8^{\pm 0.0}$ \\
\rotatebox{90}{} &  & Winkler & $1.52^{\pm 0.00}$ & $1.52^{\pm 0.00}$ \\
\cmidrule{1-5}
\multirow[c]{9}{*}{\rotatebox{90}{Air 25 PM}} & \multirow[c]{3}{*}{Forest} & $\Delta$ Cov & $-0.009^{\pm 0.000}$ & $-0.009^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $81.5^{\pm 0.0}$ & $81.4^{\pm 0.0}$ \\
\rotatebox{90}{} &  & Winkler & $2.02^{\pm 0.00}$ & $2.02^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{LGBM} & $\Delta$ Cov & $0.002^{\pm 0.001}$ & $0.001^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $73.3^{\pm 0.0}$ & $73.3^{\pm 0.0}$ \\
\rotatebox{90}{} &  & Winkler & $1.84^{\pm 0.00}$ & $1.83^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{Ridge} & $\Delta$ Cov & $0.010^{\pm 0.000}$ & $0.010^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $65.5^{\pm 0.0}$ & $65.4^{\pm 0.1}$ \\
\rotatebox{90}{} &  & Winkler & $1.40^{\pm 0.00}$ & $1.40^{\pm 0.00}$ \\
\cmidrule{1-5}
\multirow[c]{9}{*}{\rotatebox{90}{Sap flow}} & \multirow[c]{3}{*}{Forest} & $\Delta$ Cov & $0.007^{\pm 0.000}$ & $0.007^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $1743.1^{\pm 1.4}$ & $1742.7^{\pm 1.2}$ \\
\rotatebox{90}{} &  & Winkler & $0.59^{\pm 0.00}$ & $0.59^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{LGBM} & $\Delta$ Cov & $0.003^{\pm 0.000}$ & $0.003^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $1581.9^{\pm 0.7}$ & $1583.6^{\pm 1.3}$ \\
\rotatebox{90}{} &  & Winkler & $0.49^{\pm 0.00}$ & $0.49^{\pm 0.00}$ \\
\cmidrule{2-5}
\rotatebox{90}{} & \multirow[c]{3}{*}{Ridge} & $\Delta$ Cov & $-0.241^{\pm 0.000}$ & $-0.242^{\pm 0.000}$ \\
\rotatebox{90}{} &  & PI-Width & $2061.5^{\pm 1.4}$ & $2066.8^{\pm 1.2}$ \\
\rotatebox{90}{} &  & Winkler & $2.52^{\pm 0.00}$ & $2.52^{\pm 0.00}$ \\
\bottomrule
\end{tabular}
\end{table}

